Ax-Schanuel for $GL_n$

In this paper we prove an Ax-Schanuel type result for the exponential functions for general linear groups over $\mathbb{C}$. We prove the result first for the group of upper triangular matrices and then for the group $GL_n$ of all $n\times n$ invertible matrices over $\mathbb{C}$. We also obtain Ax-Lindemann type results for these maps as a corollary, characterizing the bi-algebraic subsets of these maps.

==> upper.tex <==
\textbf{Notation:} I will denote by $U=U_n$ the algebraic group of $n\times n$ upper triangular invertible matrices over the field $\mathbb{C}$, and by $\mathfrak{h}=\mathfrak{h}_n$ its Lie algebra of $n\times n$ upper triangular matrices. Also I will also denote by $E=E_n$ the corresponding exponential map $\mathfrak{h}_n\rightarrow U_n$.\\

Our first goal here is to formulate an Ax-Schanuel-type Theorem and reduce its proof to \thref{asmainred}. To that end we will prove the following

\begin{propa}\thlabel{upprop} Let $f_i,g_{i,j}\in\C[[t_1,\ldots,t_m]]$, where $1\leq i<j\leq n$, and $A=\diag(\vec{f})+(g_{i,j})$ the corresponding $n\times n$ upper triangular matrix. Let $E_{i,j}$, for $i<j$, denote the corresponding coordinate of the exponential matrix of $A$. Then \begin{center}
	$tr.d._\C\C(\{f_i,g_{i,j}, E_{i,j}, e^{f_i}:1\leq i<j\leq n\}) =tr.d._\C\C(\{f_i,g_{i,j},e^{f_i}:1\leq i<j\leq n\})$.
\end{center}




\end{propa}

\section{Calculating The Exponential}

We start with some lemmas in order to give a concrete description of the map $E$, or to be more precise a concrete enough description to answer the algebraic dependence of its coordinates $E_{i,j}$. In other words, if $A=\diag(\vec{z})+(x_{i,j})$ is an upper triangular $n\times n$ matrix, with diagonal elements $z_i$ and strictly upper triangular elements $x_{i,j}$ for $i<j$, we want to describe $E_{i,j}(A)$, the $(i,j)$ coordinate of the matrix $E(A)$, in terms of the $z_i$ and $x_{i,j}$. In order to achieve this we start by calculating the coordinates of the matrix $A^N$ in terms of the $z_i$ and $x_{i,j}$. 

In order to describe the main result of this section we will first need some definitions.

\begin{defn}Let $s,t\in \mathbb{C}$, we define the functions 
	\begin{center}
		\[F_N(s,t) = 
		\begin{cases}
		\frac{s^N-t^N}{s-t}& s\neq t\\
		N s^{N-1} & s=t\end{cases}\]
	\end{center}\begin{center}
		\[and\  F(s,t) = 
		\begin{cases}
		\frac{e^s-e^t}{s-t}& s\neq t\\
		e^s & s=t\end{cases}\]\end{center}\end{defn}
For the rest of our discussion $F$ and $F_N$ will always refer to these functions.

Momentarily, we consider the coordinates of the matrix $A\in \mathfrak{h_n}$, $z_i$ and $x_{i,j}$, as variables, for convenience, and we define $R$ to be the ring \begin{center}
	$\mathbb{Q}[x_{i,j}, \frac{1}{z_i-z_j};z_i\neq z_j,$ $i<j]$.
\end{center}
\begin{lemma}\thlabel{polylemma} Let $A\in\mathfrak{h}_n$ and $E(A)$ its exponential. Then for all $1\leq i< j\leq n$ there exists a linear polynomial $P_{i,j}[y_1,\ldots,y_{M(i,j)}] \in R[y_1,\ldots,y_{M(i,j)}]$, where $M(i,j)\in\mathbb{N}$ depends on $i,j$, such that the $(i,j)$ entry of the matrix $E(A)$ is equal to $P_{i,j}(F(z_s,z_t);\min(i,j)\leq t\leq \max(i,j), t\neq s)$, and $s=\min(i,j)$.\end{lemma}

\begin{rmks}\begin{enumerate}\item If we want to be more precise $P_{i,j}$ will be a linear combination of monomials of the form \begin{center}
			$q\prod x_{s,t}\cdot\prod\frac{1}{(z_s-z_t)}\cdot y_l$,
		\end{center} where all the $s,t$ here are integers in the interval $[\min(i,j),\max(i,j)]$, and $q\in \Q$ is some rational number. Also all the coefficients of the monomials that appear will be $\pm 1$ and each $y_l$ may appear more than once in the sum.
		\item The proof will imply that $M(i,j)=|i-j|$.
		
		\item The description of the entries $E_{i,j}$ for $i<j$ will conclude the description of the matrix $E(A)$, since its diagonal elements will be $e^{z_i}$.
\end{enumerate}\end{rmks}     

The rest of this section is dedicated to proving this lemma.\\

\textbf{The case $n=2$}\\

In order to get some better intuition for the problem in general we start by considering the simple case $n=2$. As in the general case, the first step in proving the desired result for $n=2$ will be to provide a description of the entries of the matrix $A^N$ in terms of the those of $A\in\mathfrak{h}_2$. This is the result of our first lemma. 

\begin{lemma}Let $A\in \mathfrak{h}_2$ be a random matrix, $A=\begin{pmatrix} a&x\\0&b\end{pmatrix}$, and $N\in\mathbb{N}$. Then \begin{center}
		$A^N= \begin{pmatrix}a^N&xF_N(a,b)\\0&b^N\end{pmatrix}$,
	\end{center} where $F_N(a,b)$ is as above.\end{lemma}
\begin{proof}This follows easily by induction on $N$.\end{proof}

The above lemma is the first calculation needed for the following 

\begin{lemma}\thlabel{lemmafor2} Let $A$ be as above. Then \begin{center}
		$E(A)=\begin{pmatrix}e^a&xF(a,b)\\0&e^b\end{pmatrix}$,
	\end{center} where $F(a,b)$ is as above.\end{lemma}
\begin{proof}
	Follows from the previous lemma and the formula $E(A)=\Sum{N=1}{\infty}\frac{A^N}{N!}$.
\end{proof}

\textbf{The general case}\\

We let $n\in \mathbb{N}$ and consider the map $E:\mathfrak{h}_n\rightarrow U_n$. Let $A\in \mathfrak{h}$, our first goal is to generalize the situation we had for $n=2$ and acquire a description of the entries of $A^N$ as functions of the entries of $A$. For reasons of convenience we introduce the notion of diagonal submatrix.

\begin{defn}\thlabel{defn2}Let $A$ be as above. A matrix $B\in\mathfrak{h}_k$ with $k\leq n$ will be called a \textbf{diagonal submatrix} of $A$ if \begin{center}
		$A=\begin{pmatrix}A_0&\ast&\ast\\
		0&B&\ast\\
		0&0&A_1\end{pmatrix}$,  
	\end{center} for suitable upper triangular matrices $A_0$ and $A_1$.\end{defn}


\begin{rmk}If we assume that we have solved the problem for $(n-1)\times(n-1)$ matrices then it suffices to calculate the $(1,n)$ coordinate of the matrix $A^N$. To see this start by taking any $(n-1)\times (n-1)$ diagonal submatrix $B$ of $A$ and notice that $B^N$ will be a diagonal submatrix of $A^N$ appearing in the same place in $A^N$ as $B$ in $A$. So the entries in $B^N$ will depend solely on those of $B$. 
\end{rmk}

We keep denoting by $F(s,t)$, and $F_N(s,t)$ the functions we defined in the beginning. Also, for reasons of convenience, from this point on we will denote the non-diagonal entries of our original matrix by $x_{i,j}$, for $i<j$, and the diagonal entries by $z_i$, for $1\leq i\leq n$. Considering these as variables we define once again $R$ to be the ring \begin{center}
	$\mathbb{Q}[x_{i,j}, \frac{1}{z_i-z_j};i<j]$.
\end{center} Then we want to prove the analogue of \thref{polylemma} for powers of a matrix. We start by considering matrices with distinct eigenvalues.

\begin{lemma}\thlabel{polylemman}Let $A\in\mathfrak{h}_n$ have distinct eigenvalues and $N\in \mathbb{N}$ be as above. Then for all $1\leq i< j\leq n$ there exists a linear polynomial $P_{i,j}[y_1,\ldots,y_{M(i,j)}] \in R[y_1,\ldots,y_{M(i,j)}]$, where $M(i,j)\in\mathbb{N}$ depends on $i,j$, such that the $(i,j)$ entry of the matrix $A^N$ is equal to $P_{i,j}(F_N(z_s,z_t);\min(i,j)\leq t\leq \max(i,j), t\neq s)$, and $s=\min(i,j)$.\end{lemma}


\begin{rmk}The most important fact is that the polynomial $P_{i,j}$ will be independent of the power $N$ at which we are raising. \end{rmk}


Before we start with the proof we will need the following lemma.

\begin{lemma}\thlabel{calclemma} Let $s,t,x\in \C$ and let	\begin{center}
		$x^NF_1(s,t)+x^{N-1}F_2(s,t)+\cdots+xF_{N}(s,t)+F_{N+1}(s,t)=G_N(x,s,t)$. \end{center}Then \begin{center}
		$G_N(x,s,t) =\begin{cases}\frac{1}{s-t}(F_{N+2}(s,x)-F_{N+2}(t,x))& \text{if } s\neq t\\
		\frac{x^{N+2}-x(N+2)s^{N+1}+(N+1)s^{N+2}}{(s-x)^2}&\text{if } s=t, x\neq s\\
		\frac{(N+2)(N+1)s^N	}{2}&\text{if } s=t=x
		\end{cases}.$
	\end{center}
	.
\end{lemma}
\begin{proof}The first case follows by a simple calculation. The second and third cases can be calculated as limits from the first.\end{proof}


\begin{rmk} Notice here that \begin{center}
		$G_N(x,s,t)=\begin{cases}
	\frac{F_{N+1}(x,s)}{s-x}+\frac{F_{N+1}(s,t)}{s-x}& \text{if } s=t,x\neq s\\
\frac{N+2}{2}F_{N+1}(s,x)& \text{if } s=t=x 
	\end{cases}.$
	\end{center}

\end{rmk}




In view of the remark following \thref{polylemman}, in order to prove \thref{polylemman}, it suffices to compute the $(1,n)$ entry of the matrix $A^N$. More precisely using induction and the previous remarks it suffices to prove the following lemma.

\begin{lemma}\thlabel{lemma6}Let $A\in \mathfrak{h_n}$ with $n>1$ be a matrix with distinct eigenvalues and let $H^n_N(A)$ denote the $(1,n)$ entry of the $n\times n$ matrix $A^N$. Then there exists a linear polynomial $P_{1,n}$, as in \thref{polylemman}, such that \begin{center}
		$H^n_N(A)=P_{1,n}(F_N(z_1,z_j);j\neq 1)$.
	\end{center}
\end{lemma}
\begin{proof}Assume this holds for $k\times k$ matrices for all $k\leq n$. Let $A\in\mathfrak{h}_{n+1}$. We write a recursive relation for $H_N^{n+1}$ and $H_{N+1}^{n+1}$ by computing $(1,n+1)$ in the product $A^{N+1}=A\cdot A^N$. We get 
	\begin{center} $H_{N+1}^{n+1}=z_1H^{n+1}_N+x_{1,2}H^n_N+\ldots+x_{1,n+1}H^1_N$,\end{center}
	where $H^1_N=z_{n+1}^N$, and the $H^k_r$, for $k<n+1$, will denote the entry $(1,k)$ of the matrix $B_k^r$, where $B_k$ is the $k\times k$ diagonal submatrix of $A$ that has diagonal $z_{n+2-k},\ldots, z_{n+1}$. 
	
	Continuing like this, by descending with respect to $N$, we reach the equality
	\begin{center}$H^{n+1}_{N+1}= z_1^{N+1}H_1^{n+1}+ \bigg[\Sum{j=2}{n}x_{1,j} \bigg( \Sum{k=0}{N-1}z_1^k H^{n+1-j}_{N-k}        \bigg)\bigg] +x_{1,n+1}\Sum{k=0}{N-1}z_1^kz_{n+1}^{N-k}$.
	\end{center}Finally, we use the fact that $H^{n+1}_1=x_{1,n+1}$, induction, and the result from \thref{calclemma} to get the result we wanted.\end{proof}

\begin{proof}[Proof of \thref{polylemma}] Assume first that our matrix $A$ has distinct eigenvalues. Then we note that \begin{center}$\Sum{N=1}{\infty} \frac{F_N(s,t)}{N!}=F(s,t)$.\end{center} Since the polynomials $P_{i,j}$, of \thref{polylemman}, are linear in the $F_N(z_i,z_j)$, and also independent of $N$ the result follows, with the polynomials being the same as those of \thref{polylemman}.


Let now $A\in\mathfrak{h}_n$ be a general upper triangular matrix, with $A=\diag{\vec{z}}+(x_{i,j})$. Thanks to the remark following \thref{defn2} we only need to find such a polynomial for the $(1,n)-$coordinate of $E(A)$.

We finish the proof with induction on the number $m(A)=\max\{m_i:1\leq i\leq n\}$, where $m_i$ is the multiplicity of the eigenvalue $z_i$ of $A$. For $m(A)=1$ this follows from the previous discussion. Assume it is true for $m$ and that $m(A)=m+1$.

Let $z_{i_1},\ldots,z_{i_t}$ be the distinct eigenvalues of $A$ and assume that, without loss of generality, $m_{i_1}=\ldots=m_{i_r}=m+1$. For each $1\leq s\leq r$ let $j_s=\max\{i: z_i=z_{i_s}\}$.





We can approximate $A$ by matrices $A_{\vec{k}}\in \mathfrak{h}_n$, where $\vec{k}\in\mathbb{N}^r$. We denote these matrices by $A_{\vec{k}}=\diag\vec{ z}( \vec{k} ) +(x_{i,j }(\vec{k}))$, and we may choose them so that:
\begin{enumerate}\item for all $\vec{k}$, $m(A_{\vec{k}})=m$, with $m_{i_s}(A_{\vec{k}})=m$ for $1\leq s\leq r$,
	\item for all $\vec{k}$ the $(i,j)-$th coordinate of $A_{\vec{k}}$ is equal to that of $A$ if $i<j$, i.e. $x_{i,j}=x_{i,j}(\vec{k})$ for all $\vec{k}$,
\item for all $\vec{k}$ and all $i\neq j_s$, with $1\leq s\leq r$, $z_i(\vec{k})=z_i$, and
\item for $1\leq s\leq r$ the perturbation $a_s=z_{j_s}(\vec{k})-z_{j_s}$ depends only on $k_s$ and $a_s\underset{k_s\rightarrow \infty}{\infty} 0$.\end{enumerate}
In other words we approximate $A$ by slightly perturbing the $z_{j_s}$ which increase $m(A)$.

Since the exponential is a continuous function, we get that \begin{center}$E_{1,n}(A_{\vec{k}})\underset{k_s\rightarrow \infty}{\rightarrow} E_{1,n}(A)$.\end{center} 
For $E_{1,n}(A_{\vec{k}})$ we can use the inductive hypothesis to find that \begin{equation}\label{equ1}
	E_{1,n}(A_{\vec{k}})=\frac{Q(x_{i,j},z_i(\vec{k}),e^{z_i(\vec{k})})}{\underset{(s,t)\in I}{\prod}( z_s(\vec{k})- z_t(\vec{k}))^{l(s,t)}},\end{equation}
where $I=\{(s,t):1\leq s,t\leq n, z_s(\vec{k})\neq z_t(\vec{k}) \}$, $l(s,t)$ is some natural number depending on $s,t$, and $Q$ is a polynomial with coefficients in $\Q$.

The limit as $k_s\rightarrow \infty$ of $E_{1,n}(A_{\vec{k}})$ exists, and therefore so does the limit on the right hand side of \ref{equ1}. Applying De L'Hospital we reach the conclusion.\end{proof}

\begin{proof}[Proof of \thref{upprop}] By \thref{polylemma} $E_{i,j}(A)$ can be written as a rational function on the $f_i$, $g_{i,j}$, and $e^{f_i}$. It follows that the transcendence degrees are the same.
	
	
\end{proof}	
	
	
